AgroGPT: Efficient Agricultural Vision-Language Model with Expert Tuning

Significant progress has been made in advancing large multimodal conversational models (LMMs), capitalizing on vast repositories of image-text data available online. Despite this progress, these models often encounter substantial domain gaps, hindering their ability to engage in complex conversations across new domains. Recent efforts have aimed to mitigate this issue, albeit relying on domain-specific image-text data to curate instruction-tuning data. However, many domains, such as agriculture, lack such vision-language data. In this work, we propose an approach to construct instruction-tuning data that harnesses vision-only data for the agriculture domain. We utilize diverse agricultural datasets spanning multiple domains, curate class-specific information, and employ large language models (LLMs) to construct an expert-tuning set, resulting in a 70k expert-tuning dataset called AgroInstruct. Subsequently, we expert-tuned and created AgroGPT, an efficient LMM that can hold complex agriculture-related conversations and provide useful insights. We also develop AgroEvals for evaluation and compare {AgroGPT's} performance with large open and closed-source models. {AgroGPT} excels at identifying fine-grained agricultural concepts, can act as an agriculture expert, and provides helpful information for multimodal agriculture questions. The code, datasets, and models are available at https://github.com/awaisrauf/agroGPT.

==> others/quant_results_weed.tex <==
\begin{table}
    \centering
    \begin{minipage}{0.5\textwidth}
    \resizebox{1\textwidth}{!}{
    \begin{tabular}{p{0.15\textwidth}p{0.8\textwidth}}
    \toprule
         & \includegraphics[width=0.25\textwidth]{figs/black_nightsade.jpeg}   \\
         \toprule
         \textbf{User}:     & What plant is this? Can this affect the yield of my crop? \\
         \textbf{AgroGPT}:  & The plant in the image is a {\color{blue}young black nightshade}, a weed that can negatively impact crop yields. Black nightshade competes with crops for resources and can reduce crop quality by staining and affecting the taste of produce. It is important to manage black nightshade populations to minimize its impact on agriculture. \\
         \textbf{User}:      & What are some ways to control this weed? \\
         \textbf{AgroGPT}:   & Some ways to control black nightshade include using good cropping practices, such as high seeding rates and narrow row spacing, to create dense, uniform stands that will suppress the weed. No-till systems can also help reduce nightshade densities by minimizing soil disturbance. Herbicides can be used for spot treatments, but care should be taken to avoid harming beneficial plants and to follow label instructions carefully. Solarization, which involves covering the soil with a clear film to block sunlight, can also be effective in killing nightshade seeds. \\
    \midrule
         \textbf{Bard}:      & The plant in the image is most likely a {\color{red}tomato plant (Solanum lycopersicum)}.  Depending on the variety,  tomatoes can (...)
        Whether this tomato plant will affect the yield of your crop depends on several factors, including: (...)
        If you have a large number of tomato plants, they may crowd out your other crops and reduce their yield.
        Finally, the location of the tomato plants (...)
        In general, it is best to err on the side of caution and remove any volunteer tomato plants (...). \\
    \bottomrule
    \end{tabular}}
    \end{minipage}
    \caption{Comparison of our efficient AgroGPT-3B with Google Bard on open-ended questions on a holdout image from Early Weed Detection dataset~\cite{di2017automatic}. AgroGPT-3B correctly identifies the plant as a weed harmful to crops and suggests effective control measures. In contrast, Bard incorrectly identifies the plant as a tomato and provides irrelevant suggestions.}
    \label{tab:quant_weed_test}
    \end{table}
